Safe Reinforcement Learning via Probabilistic Shields

This paper targets the efficient construction of a safety shield for decision making in scenarios that incorporate uncertainty. Markov decision processes (MDPs) are prominent models to capture such planning problems. Reinforcement learning (RL) is a machine learning technique to determine near-optimal policies in MDPs that may be unknown prior to exploring the model. However, during exploration, RL is prone to induce behavior that is undesirable or not allowed in safety- or mission-critical contexts. We introduce the concept of a probabilistic shield that enables decision-making to adhere to safety constraints with high probability. In a separation of concerns, we employ formal verification to efficiently compute the probabilities of critical decisions within a safety-relevant fragment of the MDP. We use these results to realize a shield that is applied to an RL algorithm which then optimizes the actual performance objective. We discuss tradeoffs between sufficient progress in exploration of the environment and ensuring safety. In our experiments, we demonstrate on the arcade game PAC-MAN and on a case study involving service robots that the learning efficiency increases as the learning needs orders of magnitude fewer episodes.

==> pacmantoprism.tex <==



==> pics/strategy.tex <==
\begin{tikzpicture}[label distance=-1pt]
%\node[waypoint, label={$\WPT$}] at (0.2, 4.6) {};
%\node[landmark, label={$\LM$}] at (1.1, 4.6) {};
%\node[obstacle, label={$\OBST$}] at (2.1, 4.6) {};
%\node[human={180}{green!80}, opacity=0.4, label={270:$\humaninit$}] at (3.1,4.6) {};
%\node[rectangle, fill=black!40!white, inner sep=4pt, opacity=0.5, label={Goal}] at (3.9, 4.6) {};
%\draw[fill=green!40!white, opacity=0.6] (3.9, -0.1) rectangle (4.1, 0.1);
\draw[step=1cm,gray,very thin] (0,0) grid (4,5);
\draw[fill=black!40!white, opacity=0.5] (-0.3, 4.5) rectangle (4.3, 5.5);
\node[obstacle] at (3,3) {};
\node[obstacle] at (1,1) {};
%\node[obstacle] at (0,4) {};
\node[landmark] at (1,3) {};
\node[landmark] at (4,3) {};
%%
%\node[waypoint] at (4,0) {};
\node[waypoint] at (2,1) {};
\node[waypoint] at (2,2) {};
\node[waypoint] at (2,3) {};
\node[waypoint] at (2,4) {};
\node[waypoint] at (2,5) {};
\node[waypoint] at (2,0) {};
\node[] at (-0.5,1.5) (robot) {\includegraphics[width=0.07\textwidth]{pics/marvin.png}};
\draw[green,->,very thick] (0.2,1.5) -| +(1.4,1) -| +(3.3,3);
\end{tikzpicture}


==> preliminaries.tex <==
\color{gray}
In this section, we introduce the required models and specifications considered in this paper, and provide a formal problem statement.

\paragraph{Models.}

For a set $X$, let $2^{X}$ denote the power set of $X$. 
A \emph{probability distribution} over a finite or countably infinite set $\distDom$ is a function $\distFunc\colon\distDom\rightarrow\Ireal$ with $\sum_{\distDomElem\in\distDom}\distFunc(\distDomElem)=\distFunc(\distDom)=1$. 
In this paper, all probabilities are taken from $\Q$.
Let the set of all distributions on $\distDom$ be denoted by $\Distr(\distDom)$.
The set $\supp(\distFunc)=\{x\in\distDom \mid \distFunc(x)>0\}$ is the \emph{support} of $\distFunc \in \Distr(\distDom)$. 
If $\mu(x)=1$ for $x\in\distDom$ and $\mu(y)=0$ for all $y\in\distDom\setminus\{x\}$, $\mu$ is called a \emph{Dirac distribution}.

\begin{definition}{\bf (MDP)}
A \emph{Markov decision process (MDP)} $\MdpInit$ is a tuple with a finite set $S$ of states, a unique initial state $\sinit \in S$, a finite set $\Act$ of actions, and a (partial) probabilistic transition function $\pmdp\colon S\times\Act\rightarrow\Distr(S)$.
\end{definition}
%%
MDPs operate by means of \emph{nondeterministic choices} of actions at each state, whose successors are then determined \emph{probabilistically} \wrt the associated probability distribution.
The set of \emph{enabled} actions at state $s\in S$ is denoted by $\Act(s)=\{a\in\Act\mid\exists\mu\in\Distr(S).\,\mu=\pmdp(s,\alpha)\}$. 
To avoid deadlock states, we assume that $|\Act(s)|\geq 1$ for all $s\in S$.
A \emph{cost function} $\rho\colon S\times\Act\rightarrow\R_{\geq 0}$ for an MDP $\mdp$ adds a cost to each \emph{transition} $(s,a)\in S\times\Act$ with $a\in\Act(s)$.  

A \emph{path} in an $\mdp$ is a finite (or infinite) sequence $\pi=s_0a_0s_1a_1\ldots$ with $\pmdp(s_i, \alpha, s_{i+1}) > 0$ for all $i\geq 0$. 
The set of all paths in $\mdp$ is denoted by $\pathset^\mdp$, all paths starting in state $s\in S$ by $\pathset^\mdp(s)$. 
The cost of finite path $\pi$ is defined as the sum of the costs of all transitions in $\pi$, i.e., $\rho(\pi) = \sum_{i=0}^{n-1} \rho(s_i,a_i)$ where $n$ is the number of transitions in $\pi$.

If $|\Act(s)|=1$ for all $s\in S$, all actions can be disregarded and the MDP $\mdp$ reduces to a \emph{discrete-time Markov chain (MC)}, sometimes denoted by $\dtmc$, yielding a transition probability transition function of the form $\pmdp\colon S\rightarrow\Distr(S)$.
%
%	A probability measure $\pr$ for finite paths of an MC $\dtmc$ is given by the product of transition probabilities:
%	\begin{align*}
%		\pr^\dtmc(s_0,s_1,\ldots,s_n)=\prod_{i=0}^{n-1}\pmdp(s_i)(s_{i+1})
%	\end{align*}
The \emph{unique probability measure} $\pr^\dtmc(\Pi)$ for set $\Pi$ of infinite paths of MC $\dtmc$ can be defined by the usual cylinder set construction, see~\cite{BK08} for details.
The \emph{expected cost} of the set $\Pi$ of paths, denoted by $\expRew^\dtmc(\Pi)$, is defined as $\sum_{\pi \in \Pi} \pr(\pi){\cdot}\rho(\pi)$. 

In order to define a probability measure and expected cost on MDPs, the nondeterministic choices of actions are resolved by so-called \emph{schedulers}\footnote{Also referred to as strategies or policies.}. 
As in~\cite{draeger-et-al-tacas-2014}, for practical reasons we restrict ourselves to \emph{memoryless} schedulers; more details about schedulers can be found in~\cite{BK08}.
%
\begin{definition}{\bf (Scheduler)}\label{def:scheduler}
	A \emph{scheduler} for an MDP $\mdp$ is a function $\sched\colon S\rightarrow\Distr(\Act)$ such that $\sigma(s)(a) > 0$ implies $a \in \Act(s)$. Schedulers using only Dirac distributions are called \emph{deterministic}. The set of all schedulers over $\mdp$ is denoted by $\Sched^\mdp$.
\end{definition}
%
Deterministic schedulers are functions of the form $\sched\colon S\rightarrow\Act$ with $\sigma(s) \in \Act(s)$. Schedulers that are not deterministic are also called \emph{randomized}. Applying a scheduler to an MDP yields a so-called \emph{induced Markov chain}, as all nondeterminism is resolved. 

\begin{definition}{\bf (Induced MC)}\label{def:induced_dtmc}
	Let MDP $\MdpInit$ and scheduler $\sched\in\Sched^\mdp$. The \emph{MC induced by $\mdp$ and $\sched$} is  $\mdp^\sched=(S,\sinit,\Act,\pmdp^\sched)$ where
	\begin{align*}
		\pmdp^\sched(s,s')=\sum_{a\in\Act(s)} \sched(s)(a)\cdot\pmdp(s,a)(s') \quad \mbox{ for all } s,s'\in S~.
	\end{align*} 
\end{definition}
Intuitively, the transition probabilities in $\mdp^\sched$ are obtained \wrt the random choices of action of the scheduler. 
%When reasProbabilities and expected cost on MDPs are computed based on specific schedulers on the induced MC.
%
\begin{remark}\label{rem:det_schedulers}
\emph{Deterministic schedulers} pick just one action at each state and the associated probability distribution determines the probabilities. In this case we write for all states $s\in S$ and $a\in\Act$ with $\sched(s)(a)=1$:
\begin{align*}
	\pmdp^\sched(s,s')=\pmdp(s,a)(s')\ .
\end{align*}
\end{remark}
%
%This is used to define a probability measure $\pr^{\mdp^\sched}$ \wrt specific schedulers $\sched$ for $\mdp$.

\paragraph{Specifications.}

Specifications are given by combining \emph{reachability properties} and \emph{expected cost properties}. A reachability property $\reachProplT$ with upper probability bound $\lambda\in\Irat$ and target set $T\subseteq S$ constrains the probability to finally reach $T$ from $\sinit$ in $\mdp$ to be at most $\lambda$. 
Analogously, expected cost properties $\expRewProp{\kappa}{G}$ impose an upper bound $\kappa\in\Q$ on the expected cost to reach goal states $G\subseteq S$. 
Combining both types of properties, the intuition is that a set of bad states $T$ shall only be reached with a certain probability $\lambda$ (safety specification) while the expected cost for reaching a set of goal states $G$ has to be below $\kappa$ (performance specification). 
This can be verified using multi-objective model checking~\cite{DBLP:conf/atva/ForejtKP12,DBLP:journals/lmcs/EtessamiKVY08,DBLP:conf/csl/BaierDK14}, provided all problem data (i.e., probabilities and costs) are a-priori known.

We overload the notation $\finally T$ to denote both a reachability property and the set of all paths that finally reach $T$ from the initial state $\sinit$ of an MC. The probability and the expected cost for reaching $T$ from $\sinit$ are denoted by $\pr(\finally T)$ and $\expRew(\finally T)$, respectively. Hence, $\pr^{\dtmc}(\finally T)\leq\lambda$ and $\expRew^{\dtmc}(\finally G)\leq\kappa$ express that the properties $\reachProplT$ and $\expRewProp{\kappa}{G}$ respectively are satisfied by MC $\dtmc$.

%For a set $T\subseteq S$ of target states of an MC $\dtmc$, we denote the set of finite paths starting in $s\in S$ and ending 
%in the first visit of some $t\in T$ by $\pathset^\dtmc(s,T) = 
%\{s_0 \ldots s_n \in \pathset^{\dtmc}(s) \mid s_n \in T \text{ and } s_i \notin T \text{ for all } i<n\}$.
An MDP $\mdp$ satisfies both reachability property $\varphi$ and expected cost property $\psi$, iff \emph{for all} schedulers $\sched$ it holds that the induced MC $\mdp^\sched$ satisfies the properties $\varphi$ and $\psi$, i.e., $\mdp^\sched\models\varphi$ and $\mdp^\sched\models\psi$.  In our setting, we are rather interested in the so-called \emph{synthesis problem}, where the aim is to find a scheduler $\sched$ such that both properties are satisfied (while this does not necessarily hold for all schedulers).  If $\mdp^\sched\models\varphi$, scheduler $\sigma$ is said to \emph{admit} the property $\varphi$; this is denoted by $\sched\models\varphi$.

%Furthermore, for an MDP $\mdp$, a set of goal state $G$, and a cost function $\rho$, let $\sched^*\in\Sched^\mdp$ denote a scheduler minimizing the expected cost for reaching $G$ from $\sinit$.

%	Notations:
%	\begin{itemize}
%		\item $\sched\models\varphi$, admitting reachability property $\psi=\reachProplT$ for MDP/SG
%		\item maximizing/minimizing scheduler $\sched^*_\psi$ for expected reward property $\psi=\expRewProplT$ in MDP/SG
%		\item $\sched\in\psched$ for scheduler $\sched\in\Sched$ that is ``compliant'' to permissive scheduler $\psched\in\Psched$ (see~\cite{draeger-et-al-tacas-2014})
%	\end{itemize}
%
\iffalse
Finally, there might be cases where schedulers induce loops in an MDP such that target states are not reachable any more. As this is undesired behavior in our setting, we formally fix the so-called \emph{problematic states} where this is possible. For more details, we refer to~\cite{wimmer-et-al-tcs-2014}.
\begin{definition}
	For an MDP $\MdpInit$ and a set of target states $T\subseteq S$, the set of \emph{problematic states} is given by $\probstates = \{s\in\states\mid\exists\sigma\in\Sched.\,\prob[{\mdp^{\sigma}}](\finally T) = 0\}$. The states $S\setminus\probstates$ are called \emph{unproblematic states}.
\end{definition}
\nj{Example for problematic states?}

\sj{Somewhere notice that in our context  With permissive schedulers only these demonic schedulers make sense}
\cd{Can we move this to the encoding section (if it is at all necessary to have it, that is)?}
\fi
%% Let us now state the formal problem we are facing.


\color{black}

==> table-winrates.tex <==
\begin{tabular}{@{}|r|rr|rr|rr|@{}}
\toprule
%\multicolumn{1}{|l|}{\textbf{}}                                                         & \multicolumn{1}{l|}{\textbf{}}                                                                      & \multicolumn{1}{l|}{\textbf{}}
%& \multicolumn{4}{l|}{\textbf{Total Results - Training}}                                                                                                                                                                                                                                                                                                                                   \\ \midrule
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Size,\\ \#Ghosts\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}\#Model \\ Checking\end{tabular}}} & \multicolumn{1}{c|}{\textbf{time (s)}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Score\\  w/o Shield\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Score with \\ Shield\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Win Rate \\ w/o Shield\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Win Rate \\ with Shield\end{tabular}}} \\ \midrule
%5x5,1                                                                                   & 397                                                                                                 & 29                                      & 404,9                                                                                     & 505,9                                                                                        & 0,78                                                                                         & 0,89
%\\ \midrule
%6x5,1                                                                                   & 780                                                                                                 & 48                                      & -264                                                                                     & 391                                                                                        & 0,15                                                                                         & 0,85
%\\ \midrule
9x7,1                                                                                   & 5912                                                                                                & 584                                   & -359,6                                                                                    & 535,3                                                                                     & 0,04                                                                                         & 0,84
\\ \midrule
17x6,2                                                                                  & 5841                                                                                                & 1072                                     & -195,6                                                                                    & 253,9                                                                                      & 0,04                                                                                         & 0,4
\\ \midrule
17x10,3                                                                                 & 51732                                                                                               & 3681                                   & -220,79                                                                                   & -40,52                                                                                     & 0,01                                                                                         & 0,07
\\ \midrule
27x25,4                                                                                 & 269426                                                                                              & 19941                                   & -129,25                                                                                   & 339,89                                                                                     & 0,00                                                                                          & 0,00
\\ \bottomrule
\end{tabular}

